Distributed Multi-agent Coordination over Cellular Sheaves

Techniques for coordination of multi-agent systems are vast and varied, often utilizing purpose-built solvers or controllers with tight coupling to the types of systems involved or the coordination goal. In this paper, we introduce a general unified framework for heterogeneous multi-agent coordination using the language of cellular sheaves and nonlinear sheaf Laplacians, which are generalizations of graphs and graph Laplacians. Specifically, we introduce the concept of a nonlinear homological program encompassing a choice of cellular sheaf on an undirected graph, nonlinear edge potential functions, and constrained convex node objectives, which constitutes a standard form for a wide class of coordination problems. We use the alternating direction method of multipliers to derive a distributed optimization algorithm for solving these nonlinear homological programs. To demonstrate the applicability of this framework, we show how heterogeneous coordination goals including combinations of consensus, formation, and flocking can be formulated as nonlinear homological programs and provide numerical simulations showing the efficacy of our distributed solution algorithm.

==> journal-version/cuts.tex <==
according to the following commutative diagram:
\[\begin{tikzcd}[cramped]
	{C^0(G;\mathcal{F})} & {C^1(G;\mathcal{F})} \\
	{C^0(G;\mathcal{F})} & {C^1(G;\mathcal{F})}
	\arrow["\delta", from=1-1, to=1-2]
	\arrow["{L_{\mathcal{F}}^{\nabla U}}"', from=1-1, to=2-1]
	\arrow["{\nabla U}", from=1-2, to=2-2]
	\arrow["{\delta^\ast}", from=2-2, to=2-1]
\end{tikzcd}\]


\begin{theorem}[\cite{hansen_toward_2019}]\label{thm:nonlinear-projection}
    Given a cellular sheaf $\mathcal{F}$ over $G$ and diffusivity $\alpha>0$, consider the dynamical system
    \begin{align}
    \dot{x} = -\alpha L_\mathcal{F}x.
    \label{eq:heat-equation}
    \end{align}
    \begin{enumerate}
        \item The space equilibrium points of \cref{eq:heat-equation} is the space of global sections $\Gamma(G;\mathcal{F}) = H^0(G;\mathcal{F})$.
        \item Trajectories of \cref{eq:heat-equation} initialized at $x^0 \in C^0(G;\mathcal{F})$ converge exponentially quickly to the orthogonal projection of $x^0$ onto $H^0(G;\mathcal{F})$.
    \end{enumerate}
\end{theorem}



\begin{theorem}[\cite{hansen_opinion_2021}]\label{thm:hansen-nonlinear-projection}
    Suppose $\mathcal{F}$ is a cellular sheaf over $G$ equipped with convex, differentiable, and radially unbounded edge potentials $\{U_{e}: \mathcal{F}(e) \to \mathbb{R} \}_{e \in E}$ with unique global minimum at $0$. Given diffusivity $\alpha > 0$, consider the dynamical system
    \begin{align}
        \dot{x} = -\alpha L_\mathcal{F}^{\nabla U}x.
        \label{eq:nonlinear-heat-equation}
    \end{align}
    Then, trajectories of \cref{eq:nonlinear-heat-equation} initialized at $x^0 \in C^0(G;\mathcal{F})$ converge to the orthogonal projection of $x^0$ onto $H^0(G;\mathcal{F})$.
\end{theorem}


\begin{example}[Nonconstrained Distributed Optimization]
    In a system of $N$ agents where each agent has a private convex objective function $f_i(x)$ with decision variable $x \in \mathbb{R}^k$, a ubiquitous distributed optimization problem \cite{yang_survey_2019} is to minimize the sum of each agent's cost function
    \begin{align*}
        \minimize_{x \in \mathbb{R}^k} \sum_{i = 1}^N f_i(x).
    \end{align*}
    One approach to solving this distributed optimization problem is to utilize a connected communication network $G = (V,E)$. Let $\mathcal{F} = \underline{\mathbb{R}^k}$ and $U_{e}(y) = (1/2)\|y\|^2$ for all $e \in E$. Then, $\mathsf{P} = \bigl(V,E, \underline{\mathbb{R}}, \{f_i\}, \{U_{e}\} \bigr)$ is the familiar reformulation
    \begin{equation}
    \begin{array}{ll@{}ll}
    \minimize\limits_{x \in (\mathbb{R}^k)^N} & \sum_{i\in V}f_i(x_i) \\
    \text{subject to} & (L_G \otimes I_{k \times k}) x = 0
    \end{array} \notag
\end{equation}
where the linear constraint $(L_G \otimes I_{k \times k}) x = 0$ enforces consensus.
\end{example}


\begin{remark}
    Although this ADMM algorithm can be slow to converge to high accuracy, there are several practical considerations which make the algorithm attractive nonetheless. Firstly, we can leverage the results in \cite{eckstein_douglasrachford_1992} which says that the computations of the $\mathbf{x}$ and $\mathbf{z}$ updates need not fully converge at every iteration. Rather, so long as the sum of convergence errors as $k$ tends to infinity is bounded, the overall algorithm will still converge. Secondly, although ADMM can be slow to converge to high accuracy, it typically converges to modest accuracy within tens of iterations \cite{boyd_distributed_2010}. Computing a modest accuracy solution quickly is especially useful in online control contexts such as model predictive control.
\end{remark}


\begin{remark}
    When potential functions are chosen that violate Assumption \ref{as:quad-potentials}, the same ADMM algorithm can still be used to solve the relaxed problem \eqref{eq:prob-relaxation} with slight modification to the $\mathbf{z}$ update. The $\mathbf{z}$ update changes to computing a minimizer of $U(\delta_\FF \mathbf{z}) + (\rho/2)\|\mathbf{x}^{k+1} - \mathbf{z} + \mathbf{y}^k\|_2^2$. In the case of the fixed distance potential function, such a minimizer can still be computed locally.
\end{remark}

% APPENDIX

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\appendix
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{proof}[Proof of \cref{thm:hp-convexity}]
    Because each $f_i$ is convex and the sum of convex functions is convex, the objective is clearly convex. It remains to show that the constraint set $\mathcal{C}=\{x\mid L_\mathcal{F}^{\nabla U}x=0\}$ is convex. For this, we utilize the fact that $L_\mathcal{F}^{\nabla U}$ is the gradient of the function $g(x) = U(\delta_\mathcal{F} x)$. This function is clearly differentiable and is convex because the precomposition of a convex function with a linear map is convex (\cite{theRock}, Theorem 5.7). Thus we can apply Theorem 23.5 of \cite{theRock} to obtain the following
    \[
    x'= \nabla g(x)\iff x\in \partial g^*(x'),
    \]
    where $\partial$ denotes the subdifferential and $g^*$ is the Legendre transform of $g$.
    Instantiating the above with $x'=0$, we see that the set $\{x\mid \nabla g(x)=0\}$ is equivalent to the set $\{x\mid x\in \partial g^*(0)\}$. The set of subgradients of a convex function at any point is closed and convex, therefore, the set $\mathcal{C}$ is closed and convex. So $\mathsf{P}$ asks to minimize a convex function restricted to a closed convex subset of its domain and is therefore a convex optimization problem.
\end{proof}

\begin{proof}[Proof of \cref{thm:nonlinear-projection}]
    For notational convenience, we let $L=L_\FF^{\nabla U}$ and $\delta=\delta_\FF$ for the remainder of the proof.
    First note that plainly $b$ is the unique global minimizer of $U$, and $U(b)=0$. Thus $\nabla U(y)=0$ only when $y=b$. The rest of this proof proceeds similarly to that of Theorem \ref{thm:linear-projection}  \sam{Fix this!!!!} while accounting for the minimizer of $U$ being $b$ instead of 0. Specifically, we know that $L= \nabla(U\circ\delta)= \delta^\top\circ\nabla U \circ\delta$. This entails that $\dot{x}$ is always in $\image\delta^\top$ and therefore orthogonal to $\ker\delta$. We thus decompose $x$ as $x^{||} + x^\perp$ where $x^{||}$ is the orthogonal projection onto $\ker\delta=H^0(G;\FF)$ and focus on the evolution of $x^\perp$ under the dynamics restricted to $\image\delta^\top$.

    Let $\Psi(x^\perp)=U(\delta x^\perp)$. Because $b$ is the unique minimizer of $U$ with $U(b)=0$, $\Psi$ vanishes only at $\delta x^\perp =b$. Moreover, $\delta x^\perp = b$ holds if and only if $x^\perp = \delta^+b$. To show the first direction of this implication, we have
    \[
    \delta x^\perp=b \implies \delta^+\delta x^\perp = \delta^+b\implies x^\perp=\delta^+b,
    \]
    where the second implication holds because $\delta^+\delta$ is projection onto $\image \delta^\top$ and is therefore the identity on $x^\perp$. For the reverse direction, we have
    \[
    x^\perp =\delta^+b\implies \delta x^\perp=\delta\delta^+ b\implies \delta x^\perp = b,
    \]
    where the second implication holds because $\delta\delta^+$ is projection onto $\image \delta$ and is therefore the identity on $b$.

    So, $\Psi(x^\perp)$ vanishes only when $x^\perp = \delta^+b$ implying that $\nabla\Psi(x^\perp)=L(x^\perp)=0$ if and only if $x^\perp=\delta^+b$ and that $\Psi(x^\perp)$ is globally positive definite about $\delta^+b$. Furthermore, radial unboundedness of $U$ implies radial unboundedness of $\Psi(x^\perp)$. Finally, we see that
    \[
    \dot{\Psi}=\langle\nabla\Psi(x^\perp), \dot{x^\perp}\rangle = \langle L(x^\perp), -\alpha L(x^\perp)\rangle \leq 0
    \]
    with equality only when $x^\perp=\delta^+b$. This shows the $\dot{\Psi}$ is globally negative definite around $\delta^+b$, meaning $\Psi$ is a global Lyapunov function about $\delta^+b$ for the dynamics in \eqref{eq:nonlinear-diffusion-dynamics} restricted to $\image \delta^\top$. Therefore $\delta^+b$ is globally asymptotically stable meaning $x^\perp\to\delta^+ b$. For the unrestricted dynamics in \eqref{eq:nonlinear-diffusion-dynamics}, this means 
    \[\underset{t\to\infty}{\lim} x(t) = x^{||}(0) + \delta^+ b,\]
    which is orthogonal projection of $x(0)$ onto $\delta^+b+\ker\delta=\delta^+b + H^0(G;\FF)$.

    To finish the proof, it remains to show that $\delta^+b + H^0(G;\FF) = \ker L$. For the first direction, let $z\in \delta^+b + \ker\delta$. Then we know $z$ is of the form $\delta^+b + x$ for some $x$ such that $\delta x=0$. We have
    \[
    \begin{array}{ll@{}ll}
    L(z) &= \delta^\top(\nabla U(\delta(\delta^+b+x)))\\ &= \delta^\top(\nabla U(\delta\delta^+ b +\delta x)) = \delta^\top(\nabla U(b))=0,
    \end{array}
    \]
    where the third equality holds because $\delta\delta^+$ is projection onto $\image \delta$ and $x\in\ker \delta$. For the reverse direction, let $L(x)=0$ for some $x$. We know that this only holds when $\delta x=b$ which implies that $\delta^+\delta x = \delta^+b$. Because $\delta^+\delta$ is projection onto $\image\delta^\top = (\ker\delta)^\perp$, we know that $x$ must be of the form $\delta^+b + x'$ for some $x'\in\ker \delta$. This completes the proof.
\end{proof}

